Ignore or Comply? On Breaking Symmetry in Consensus

We study consensus processes on the complete graph of $n$ nodes. Initially, each node supports one from up to n opinions. Nodes randomly and in parallel sample the opinions of constant many nodes. Based on these samples, they use an update rule to change their own opinion. The goal is to reach consensus, a configuration where all nodes support the same opinion. We compare two well-known update rules: 2-Choices and 3-Majority. In the former, each node samples two nodes and adopts their opinion if they agree. In the latter, each node samples three nodes: If an opinion is supported by at least two samples the node adopts it, otherwise it randomly adopts one of the sampled opinions. Known results for these update rules focus on initial configurations with a limited number of colors (say $n^{1/3}$ ), or typically assume a bias, where one opinion has a much larger support than any other. For such biased configurations, the time to reach consensus is roughly the same for 2-Choices and 3-Majority. Interestingly, we prove that this is no longer true for configurations with a large number of initial colors. In particular, we show that 3-Majority reaches consensus with high probability in $O(n^{3/4}\log^{7/8}n)$ rounds, while 2-Choices can need $\Omega(n/\log n)$ rounds. We thus get the first unconditional sublinear bound for 3-Majority and the first result separating the consensus time of these processes. Along the way, we develop a framework that allows a fine-grained comparison between consensus processes from a specific class. We believe that this framework might help to classify the performance of more consensus processes.

==> trunk/drift_theorems.tex <==
In this section we generalize the drift theorems of \cite{LS16,J10,HY01}.
%
The drift theorems we are aware of give bounds of the form $\hat T=\min \{ t\geq 0
~|~ X_t=0\}$, for some random variable $\E{X_t-X_{t-1}}$ is negative. We extend existing drift theorem  theorems to allow to bound
stopping times $T$ of the kind  $T=\min \{ t\geq 0 ~|~ X_t\leq k\}$ for
some $k\in \mathbb{N}$.
%
Our goal is to prove the variable \autoref{vardrift} which is a straight-forward generalization
of \cite[Theorem~2]{LS16}, when one is interested in when
the given process goes below a certain threshold rather than when it reaches state 0.
It requires a slightly more general version of the additive drift theorem which we present in the following.
The proof of the additive drift theorem is a well-known simple application of the optional stopping theorem where we require that (i) $\E{X_t-X_{t-1}}$ is negative and that
$\E{X_T-X_{T-1}}$ is bounded away from $0$.


\begin{lemma}[Additive Drift] \label{adddrift}
    Let $(X_t)_{t \geq 0}$ be a Markov chain with state space $\mathcal{S}=  [
    0,\infty)$ with $X_0 = m$. Let $k,k'\in \mathcal{S}$, $k'\leq k$. Let $T$ be the random
    variable that denotes the earliest point in time $t \geq 0$ such that $X_t
    \leq k$.
    %
    Suppose the following hold:
    \begin{enumerate}
        \item $\E{X_T} \geq k' $
        \item $\E{T}$ is finite.
        \item There exists $c >0$ such that for all $x \in \mathcal{S}$, $x> k$ we have
            \[
                \E{X_{t+1}~|~X_t = x }\leq x-c.
            \]
    \end{enumerate}
    Then, $ \E{T}\leq  \frac{m-k'}{c}.$
\end{lemma}
%
\begin{proof}
	Hypothesis 3 implies $\E{X_{t+1}~| T>t }=\E{X_{t}~| T>t } -c$.
	Let $\mathcal{F}_t$ be the filtration corresponding to the histories of $X_t$ up to time $t$.
	Let $Y_t = X_{ \min\{t,T\} }+ c\cdot \min\{t,T\}$, and observe that $Y_t$ is a super-martingale.
	\begin{align}
		\E{ Y_{t+1} ~|~\mathcal{F}_t}
        &=   \E{  X_{ \min\{t+1,T\} } + c\cdot \min\{t+1,T\}~|~\mathcal{F}_t} \\
        &= \E{  X_{ \min\{t+1,T\} }   ~|~\mathcal{F}_t}+ c\cdot \min\{t+1,T\}\\
		&\leq  \E{  X_{ \min\{t,T\} } -c\cdot \mathds{1}_{T>t}   ~|~\mathcal{F}_t}+ c\cdot \min\{t+1,T\}\\
		&\leq  X_{ \min\{t,T\} }+ c\cdot \min\{t+1,T\}  -c\cdot \mathds{1}_{T>t}\\
		&= Y_t,
        \label{eq:first_drift}
	\end{align}
    where we distinguish between the cases $T\geq t+1$ and $T\leq t$.
     %
	Since $\E{T}$ is finite, from the optional stopping theorem we get
    \begin{align}
        m = \E{Y_0}
        & \geq \E{Y_T}\\
        & \stackrel{\eqref{eq:first_drift}}{=} \E{X_T} + c\cdot \E{T} \\
        & \!\!\!\! \stackrel{\text{Hyp.~1}}{\geq} k'  + c\cdot \E{T}.
    \end{align}
	Rearranging the terms yields $\E{T} \leq (m-k')/c$, concluding the proof.
\end{proof}

\begin{lemma}[Variable Drift]
    \label{vardrift}
    Let $(X_t)_{t \geq 0}$ be a Markov chain with state space $\mathcal{S}= \{
    0 \} \cup [1,\infty)$ and with $X_0 = m$. Let $k,k'\in \mathcal{S}$. Let $T$ be
    the random variable that denotes the earliest point in time $t \geq 0$
    such that $X_t \leq k$. Suppose that the following hold:
    %
    \begin{enumerate}
        \item $X_T \geq k' $.
        \item $\E{T}$ is finite.
        \item  There exists a positive, increasing function $h : \mathbb{N}
            \rightarrow \mathbb{R}_{>0}$ such that for all $x \in \mathcal{S}$,
            $x > k$ we
            have
            \begin{equation}
                \E{X_{t+1}~|~X_t = x }\leq x-h(x) .
                \label{eq:drift_h}
            \end{equation}
    \end{enumerate}

    Then $$ \E{T}\leq  \int\limits_{k'}^{m} \frac{1}{h(u)} du.$$
\end{lemma}
%
\begin{proof}
	Define
    \[
        g(x)=
        \begin{cases}
            \frac{1}{h(1)} + \int\limits_{1}^{x}  \frac{1}{h(u)} du ~&~\text{for $x\in \mathcal{S}, x>0$}\\
            0~&~\text{otherwise}.
        \end{cases}
    \]
    We first show that $g(x) - g(y) \geq (x-y)/h(x)$ for all $x,y\in
    \mathbb{N}$ with $x\geq y >0$. To see this, observe that, using that
    $h(\cdot)$ is positive and increasing,
    \begin{equation}
        g(x)-g(y)=
        \begin{cases}
             \int\limits_{y}^{x}  \frac{1}{h(u)} du \geq (x-y)/h(x) ~&~\text{for $x\geq y
             >0$}\\
            \frac{1}{h(1)} + \int\limits_{1}^{x}  \frac{1}{h(u)} du \geq x/h(x)~&~\text{for $x>y=0$}\\
        \end{cases}
        \label{eq:drift_g_def}
    \end{equation}
	We define the random variable $Y_t=g(X_t)$.
    %
    For each $x>k$ and $y=g(x)$ we have
	\begin{align} 
        \E{Y_{t}-Y_{t+1}~|~Y_t=y} 
        & \stackrel{\eqref{eq:drift_g_def}}{=} \E{g(X_{t})-g(X_{t+1})~|~X_t=x} \\
        & \stackrel{\eqref{eq:drift_h}}{\geq} \E{\frac{X_t-X_{t+1}}{h(x)}~|~X_t=x} 
            \geq 1.
	\end{align}
	Thus, for each $y>g(k)$ we have
    \begin{equation}
        \E{Y_{t+1}~|~Y_t=y} \leq y -1.
        \label{eq:second_drift_thm_additive_cond}
    \end{equation}
    
    We now observe that $Y_t$ satisfies the hypotheses of \autoref{adddrift}:
    \begin{enumerate}
        \item[1.] From Hypothesis 1 (of the present lemma) and the
            monotonicity of $g$ it follows that ${Y_T}\geq g(k')$, which
            implies $\E{Y_T}\geq g(k')$.
        \item[2.] From the monotonocity of $g$ it also follows that
            $T=\min \{ t \geq 0~|~ X_t \leq k\}= \min\{ t \geq 0~|~ Y_t \leq
            g(k)\}$, i.e. $T$ is also the earliest time such that $Y_t \leq
            g(k)$, and $\E{T}$ is finite by Hypothesis 2.
        \item[3.] The third hypothesis of \autoref{adddrift} is given by
            \eqref{eq:second_drift_thm_additive_cond}.  
    \end{enumerate}
    %
    Finally, by applying \autoref{adddrift}, we get 
    \[
        \E{T}\leq  {g(m)-\E{g(X_T)}}
            \leq g(m)-g(k') =\int\limits_{k'}^{m} \frac{1}{h(u)} du,
    \]
	concluding the proof.
\end{proof}


